An Exploratory Study of Debugging Episodes

Many studies have long investigated how developers debug, shaping our understanding of debugging and helping motivate the creation of more effective tools. However, less is known about the typical progression of debugging in real world settings. In this study, we focus on characterizing debugging episodes from the moment at which developers first encounter a defect to the moment at which it is resolved. We investigate the typical duration and frequency of debugging episodes and the typical activities which occur. We observed developers by watching professional developers at work in live-streamed programming sessions. Using this data source, we curated 15 sessions in which 11 professional developers worked for 30 hours. We then systematically coded the debugging episodes and activities that occurred within these videos, yielding a dataset of 2137 debugging activities and 1407 programming activities. We found that debugging was frequent, even in programming work, occurring once every eight minutes. Debugging episodes vary greatly in time, with most being less than a few minutes and a few as more than 100 minutes. However, most debugging time is spent in long debugging episodes. We found no single activity that dominated debugging time, and long debugging episodes often involved many diverse activities. Finally, we found that,in terms of the activities developers did, programming and debugging were remarkably similar, particularly in the frequency of editing and browsing code.

==> tables/oldOverallTable.tex <==

{\renewcommand*{\thefootnote}{\fnsymbol{footnote}}
\begin{table*}[]
\centering
\caption{A summary of the characteristics of each debugging activity. Some these characteristic are related to instances of the activities (denoted by{\footnotesize{*}}) and other are related to debugging episodes (denoted by{\footnotesize{$^\$$}})}
\label{tab:summeryActivities}
\begin{tabular}{lllllllll}
       \hline
             %   Activities
            \multicolumn{3}{c}{Browsing A File}                     
            & \multicolumn{3}{c}{Editing A File}                    
            & \multicolumn{3}{c}{Testing Program}                   
            \\
                % \multicolumn{3}{c}{{\scriptsize Looking at a file of code without introducing any change}} & 
                % \multicolumn{3}{c}{{\scriptsize Changing the source inside a file}}  & 
                % \multicolumn{3}{c}{{\scriptsize Running programs to observe final output}}                   
                % \\  
                \hline
                Avg occurrence{\footnotesize{$^\$$}} & \multicolumn{2}{l}{7 ($\pm$14)}  & 
                Avg occurrence{\footnotesize{$^\$$}} & \multicolumn{2}{l}{7 ($\pm$10)}  &               
                Avg occurrence{\footnotesize{$^\$$}} & \multicolumn{2}{l}{6 ($\pm$6)}  
                \vspace{3pt} 
                \\
              
                 Occurrence density{\footnotesize{$^\$$}} & \multicolumn{2}{l}{\includegraphics[scale=.035, trim = 5cm 8cm 10cm 4cm]{figures/browsing.png}}&     
                 Occurrence density{\footnotesize{$^\$$}} & \multicolumn{2}{l}{\includegraphics[scale=.035, trim = 5cm 8cm 10cm 4cm]{figures/editing.png}}&     
                 Occurrence density{\footnotesize{$^\$$}} & \multicolumn{2}{l}{\includegraphics[scale=.035, trim = 5cm 8cm 10cm 4cm]{figures/testing.png}}   
                 \vspace{3pt} 
                 \\ 
                
                Avg occupancy{\footnotesize{$^\$$}} & \multicolumn{2}{l}{12\% ($\pm$12\%)}     &
                Avg occupancy{\footnotesize{$^\$$}} & \multicolumn{2}{l}{40\% ($\pm$21\%)}     &
                Avg occupancy{\footnotesize{$^\$$}} & \multicolumn{2}{l}{32\% ($\pm$22\%)}    
                \vspace{3pt} 
                \\
                \multirow{2}{*}{Avg number of files{\footnotesize{$^\$$}}}  & \multicolumn{2}{l}{\multirow{2}{*}{3 ($\pm$5)}} & 
                \multirow{2}{*}{Avg number of files{\footnotesize{$^\$$}}} & \multicolumn{2}{l}{\multirow{2}{*}{2 ($\pm$2)}} & 
                \multirow{2}{*}{Testing methods{\footnotesize{*}}}  & Manual   & 84\% \\& \multicolumn{2}{l}{}& & \multicolumn{2}{l}{}&& 
                                      Unit test  & 16\%
                                      \vspace{3pt} 
              \\
                Avg time{\footnotesize{*}} & \multicolumn{2}{l}{14{\small s} ($\pm$21{\small s})}     &
                Avg time{\footnotesize{*}} & \multicolumn{2}{l}{33{\small s} ($\pm$63{\small s})}     &
                Avg time{\footnotesize{*}} & \multicolumn{2}{l}{22{\small s} ($\pm$26{\small s})}
                \vspace{3pt} 
                \\
            \multirow{3}{*}{Type of files{\footnotesize{*}}} & Source code & \multicolumn{1}{l}{85\%}& 
            \multirow{3}{*}{Type of files{\footnotesize{*}}} & Source code       & \multicolumn{1}{l}{84\%}      &
            \multirow{2}{*}{Testing targets{\footnotesize{*}}} & Current Program  & 98\% \\
            & Test  & \multicolumn{1}{l}{7\%} &                  
            & Test & \multicolumn{1}{l}{8\%} &      
            & Other programs        & 2\%       \\
            & Config & \multicolumn{1}{l}{8\%} &                   
            & Config & \multicolumn{1}{l}{8\%} & & &     
            \vspace{3pt} 
            \\
            && \multicolumn{1}{l}{} 
            & \multirow{2}{*}{Type of edit{\footnotesize{*}}} & Behaviour  & \multicolumn{1}{l}{94\%} &&& \\
            & & \multicolumn{1}{l}{}& & Instrumental & \multicolumn{1}{l}{6\%} &&& \\
                  \hline
                  
                %   Activities
            \multicolumn{3}{c}{Inspecting program state}&
            \multicolumn{3}{c}{Consulting external resources} & 
            \multicolumn{3}{c}{Other} 
            \\
            % \multicolumn{3}{c}{{\scriptsize Running program to observe intermediate state}} &
            % \multicolumn{3}{c}{{\scriptsize Searching for information outside the development environment}}&
            % \multicolumn{3}{c}{{\scriptsize Engaging in non-coding focus activities}}                     
            % \\ 
                \hline
                Avg occurrence{\footnotesize{$^\$$}} & \multicolumn{2}{l}{2 ($\pm$14)}  & 
                Avg occurrence{\footnotesize{$^\$$}} & \multicolumn{2}{l}{1 ($\pm$2)}  &               
                Avg occurrence{\footnotesize{$^\$$}} & \multicolumn{2}{l}{2 ($\pm$5)}  
                \vspace{3pt} 
                \\
                 Occurrence density{\footnotesize{$^\$$}} & \multicolumn{2}{l}{\includegraphics[scale=.035, trim = 5cm 8cm 10cm 4cm]{figures/debugging.png}}&     
                 Occurrence density{\footnotesize{$^\$$}} & \multicolumn{2}{l}{\includegraphics[scale=.035, trim = 5cm 8cm 10cm 4cm]{figures/consulting.png}}&     
                 Occurrence density{\footnotesize{$^\$$}} & \multicolumn{2}{l}{\includegraphics[scale=.03, trim = 5cm 10cm 10cm 4cm]{figures/others.png}}  
                 \vspace{3pt} 
                   \\ 
                Avg occupancy{\footnotesize{$^\$$}} & \multicolumn{2}{l}{8\% ($\pm$14\%)}     &
                Avg occupancy{\footnotesize{$^\$$}} & \multicolumn{2}{l}{3\% ($\pm$10\%)}     &
                Avg occupancy{\footnotesize{$^\$$}} & \multicolumn{2}{l}{4\% ($\pm$8\%)}   
                \vspace{3pt} 
                \\
                Avg time{\footnotesize{*}} & \multicolumn{2}{l}{53{\small s} ($\pm$105{\small s})}     &
                Avg time{\footnotesize{*}} & \multicolumn{2}{l}{35{\small s} ($\pm$42{\small s})}     &
                Avg time{\footnotesize{*}} & \multicolumn{2}{l}{22{\small s} ($\pm$24{\small s})}
                \vspace{3pt} 
                \\
                \multirow{2}{*}{Methods{\footnotesize{*}}} & 
                Log & \multicolumn{1}{l}{70\%} &
                \multirow{3}{*}{Type of resources{\footnotesize{*}}}& 
                Documentation& \multicolumn{1}{l}{83\%}&
                \multirow{3}{*}{Type of activities{\footnotesize{*}}}&
                Issue tracker & 15\% \\
                 & Debugger  & \multicolumn{1}{l}{30\%}  &
                 & Code examples  & \multicolumn{1}{l}{9\%} &
                 & Taking notes & 3\%  \\
                 &    & \multicolumn{1}{l}{}   & 
                 & Q\&A communities & \multicolumn{1}{l}{19\%} &
                 & Interact with IDE & 74\% 
                 \vspace{3pt} 
                \\
                &    & & \multirow{2}{*}{Initiation{\footnotesize{*}}} & Explanation of error & 8\%                    
                 & &  &  \\
                 & & &                     
                 & Explanation of API & 92\% & & &  
                 \\
 \hline
    %   \multicolumn{4}{r}{\footnotesize{$^\$$ Across debugging episodes}} & \multicolumn{3}{l}{\footnotesize{$^*$ Across instances of the activity}}

\end{tabular}
\end{table*}
}


